Histology to 3D In Vivo MR Registration for Volumetric Evaluation of MRgFUS Treatment Assessment Biomarkers

Advances in imaging and early cancer detection have increased interest in magnetic resonance (MR) guided focused ultrasound (MRgFUS) technologies for cancer treatment. MRgFUS ablation treatments could reduce surgical risks, preserve organ tissue/function, and improve patient quality of life. However, surgical resection and histological analysis remain the gold standard to assess cancer treatment response. For non-invasive ablation therapies such as MRgFUS, the treatment response must be determined through MR imaging biomarkers. However, current MR biomarkers are inconclusive and have not been rigorously evaluated against histology via accurate registration. Existing registration methods rely on anatomical features to directly register in vivo MR and histology. For MRgFUS applications in anatomies such as liver, kidney, or breast, anatomical features independent from treatment features are often insufficient to perform direct registration. We present a novel MR to histology registration workflow that utilizes intermediate imaging and does not rely on these independent features. The presented workflow yields an overall registration accuracy of 1.00 +/- 0.13 mm. The developed registration pipeline is used to evaluate a common MRgFUS treatment assessment biomarker against histology. Evaluating MR biomarkers against histology using this registration pipeline will facilitate validating novel MRgFUS biomarkers to improve treatment assessment without surgical intervention.

==> Figures/imaging_parameters/imaging_param_table.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[ht]
	\centering
	\ra{1.3}
	\small
	\caption{\label{tab:params}Parameters for the multiparametric scanning sequence used for ablation day and follow-up imaging. Coronal orientation was used for all MR acquisitions. TR: Repetition Time, TE: Echo Time, EPI: Echo Planar Imaging, SPACE: Sampling Perfection with Application Optimized Contrasts Using Different Flip Angle Evolution, VIBE: Volumetric Interpolated Breath-Hold, GRE: Gradient Recalled Echo, MRTI: Magnetic Resonance Temperature Imaging, SS: Single Shot, SE: Spin Echo, and ETL: Echo Train Length. $^{*}$ T1w sequence with contrast for NPV segmentation. $^{**}$ T1w sequence without contrast for image registration. }
	\begin{tabular}{@{}l c c c c c c c c@{}} \toprule
		Stage & TR (ms) & TE (ms) & \begin{tabular}
			{@{}c@{}}Field of \\View (mm)
		\end{tabular}  &   \begin{tabular}
			{@{}c@{}}Pixel Bandwidth \\ (Hz/Pixel)
		\end{tabular} &   Resolution (mm)\\ \midrule
		\textit{in vivo} MR & 25 & 11 & 192$\times$150$\times$20 & 750 & 1.5$\times$1.5$\times$2.0\\
		\textit{ex vivo} MR & 7.19 & 2.05 & 256$\times$192$\times$52 & 250 & 1.0$\times$1.0$\times$1.0\\
		Blockface & 2000 & 300 & 256$\times$192$\times$52 & 700 & 1.0$\times$1.0$\times$1.0\\
		Microscopy & 7.19 & 2.52 & 256$\times$192$\times$56 & 250 & 0.5$\times$0.5$\times$1.0\\  \bottomrule
	\end{tabular}
\end{table*} %MR parameters

==> Figures/projection/projection_bar_plot.tex <==
% \definecolor{cat1_color}{RGB}{112,39,195}%
% \definecolor{cat2_color}{RGB}{150,0,205}%
% \definecolor{cat3_color}{RGB}{181,100,227}%
% \definecolor{cat4_color}{RGB}{236,71,233}%
% \makeatletter
% \newcommand\resetstackedplotsfive{
% \makeatletter
% \pgfplots@stacked@isfirstplottrue
% \makeatother
% \addplot [forget plot,draw=none] coordinates{(1,0) (2,0) (3,0) (4,0) (5,0)};
% }
% \begin{figure}[tb]
% \centering
% \begin{minipage}{0.49\textwidth}
%     \centering
% \begin{tikzpicture}
% \tikzstyle{every node}=[font=\small]
% \begin{axis}[
%     width=0.9\columnwidth,
%     scale only axis=true,
%     height=5cm,
%     xtick={1,...,4},
%     xticklabels={1,2,3,4},
%     enlarge x limits=0.2,
%     ymajorgrids,
%     major tick length = 0,
%     ylabel = TRE (mm),
%     ymax=1.8,
%     xlabel={Subject Number},
%     % ybar=1pt,
%     ybar stacked,
%     % symbolic x coords={s1r, s1a, s2r, s2a, s3r, s3a, s4r, s4a}
%     legend style={at={(0.5,0.97)},anchor=north, legend cell align=left, align=left, draw=black}, legend columns=2
%     ]
% \addplot[
%     fill=cat2_color,
%     draw=black,
%     point meta=y,
%     every node near coord/.style={inner ysep=5pt},
%     error bars/.cd,
%         y dir=both,
%         y explicit
% ] 
% table [x=num, y error=r2ds, y=r2dm, col sep=comma] {Figures/projection/stats.csv};
% \addlegendentry{R2 Error}
% \addplot[
%     fill=cat4_color,
%     draw=black,
%     point meta=y,
%     every node near coord/.style={inner ysep=5pt},
%     error bars/.cd,
%         y dir=both,
%         y explicit,
% ] 
% table [x=num, y error=ffzas, y=ffzam, col sep=comma] {Figures/projection/stats.csv};
% \resetstackedplots
% \addplot[
%     fill=cat4_color,
%     draw=black,
%     point meta=y,
%     every node near coord/.style={inner ysep=5pt},
%     error bars/.cd,
%         y dir=both,
%         y explicit,
% ] 
% table [x=num, y error=ffzas, y=ffzam, col sep=comma] {Figures/projection/stats.csv};
% \addplot[
%     fill=cat4_color,
%     draw=black,
%     point meta=y,
%     every node near coord/.style={inner ysep=5pt},
%     error bars/.cd,
%         y dir=both,
%         y explicit,
% ] 
% table [x=num, y error=fftas, y=fftam, col sep=comma] {Figures/projection/stats.csv};
% \addlegendentry{R1 Error \hspace{5mm}} 
% \draw ({rel axis cs:0,0}|-{axis cs:0,0}) -- ({rel axis cs:1,0}|-{axis cs:0,0});
% \end{axis}
% \end{tikzpicture}
% \end{minipage}
%     \caption{Plot of the TRE for the different stages of the registration pipeline for each subject.}
%     \label{fig:TRE}
% \end{figure} % TRE bar plot

% \makeatletter
% \newcommand\resetstackedplotsfive{
% \makeatletter
% \pgfplots@stacked@isfirstplottrue
% \makeatother
% \addplot [forget plot,draw=none] coordinates{(1,0) (2,0) (3,0) (4,0)};
% }
% \definecolor{cat1_color}{RGB}{0,48,143}%
% \definecolor{cat2_color}{RGB}{25,116,210}%
% \definecolor{cat3_color}{RGB}{255,162,186}%
% \definecolor{cat4_color}{RGB}{223,41,32}%
% \begin{filecontents}{data.csv}
% X   N   Name    Activation  Inclusion   Min     Max
% .85   3   CR      0.2125        0.0000        0.0694    0.0694
% 1.15   3   LR      0.5480        0.6415        0.4714    0.4714
% 1.85   5   CR      0.2171        0.0000        0.0296    0.0296
% 2.15   5   LR      0.4895        0.3736        0.2392    0.2392
% 2.85   7   CR      0.2212        0.0000        0.0240    0.0240
% 3.15   7   LR      0.4350        0.2249        0.4327    0.4327
% 3.85  9   CR      0.3211        0.0000        0.1834    0.1834
% 4.15  9   LR      0.4374        0.2083        0.6630    0.6630
% \end{filecontents}
% \def\datafile{data.csv}

\begin{figure}[tb]
\centering
\begin{minipage}{0.49\textwidth}
    \centering
\begin{tikzpicture}
\begin{axis}[set layers,
    % axis lines*=left,
    width=.9\columnwidth,
    % scale only axis=true,
%     height=5cm,
%     xtick={1,...,4},
%     xticklabels={1,2,3,4},
    % enlarge x limits=0.0,
%     ymajorgrids,
    major tick length = 0,
    ylabel = TRE (mm),
    xlabel={Subject Number},
    ymajorgrids,
    % width=.8\linewidth, 
    height=5cm,
    ymin=-.1,
    ymax=1.7,
    xticklabels={1,2,3,4},
    % ytick={0,2,4,6,8,10},
    ybar stacked,
    % bar width=14.7pt,
    xtick={1,2,3,4},
    legend style={at={(0.5,0.97)},anchor=north, legend cell align=left, align=left, draw=black},
    % xticklabels={3,5,7,9,11},
    legend columns=2
]
\addplot
    [forget plot, fill=cat2_color, discard if={Name}{LR}]
    table [x=X, y=Activation] {\datafile};
\addplot
    [
    on layer=axis foreground,
    fill=cat2_color, discard if={Name}{LR},
    error bars/.cd, y dir=both, y explicit,
    ]
    table [x=X, y=Inclusion, y error plus=Max, y error minus=Min] {\datafile};
\addlegendentry{R2 Error \hspace{1mm}}
\resetstackedplotsfive
\addplot
    [black, fill=cat4_color, discard if={Name}{CR}]
    table [x=X, y=Activation] {\datafile};
\addplot
    [on layer=axis foreground,
    fill=cat3_color, discard if={Name}{CR}, error bars/.cd, y dir=both, y explicit,]
    table [x=X, y=Inclusion, y error plus=Max, y error minus=Min] {\datafile};
\addplot
    [
    on layer=axis foreground,
    fill=cat2_color, discard if={Name}{LR},
    error bars/.cd, y dir=both, y explicit
    ]
    table [x=X, y=Inclusion] {\datafile};
\addlegendentry{2D Slice}
\end{axis}
\end{tikzpicture}
\end{minipage}
\caption{Subject specific plot of the TRE from \textit{ex vivo} registration for the proposed method versus the 2D slice correlation method. The dark region of the 2D slice bar shows the portion of the total error resulting only from the Z dimension. The proposed method is significantly better than the total error and the error from only the Z dimension.  }
\label{fig:projection}
\end{figure}



